Convergence of the Preconditioned Proximal Point Method and Douglas-Rachford Splitting in the Absence of Monotonicity

The proximal point algorithm (PPA) is the most widely recognized method for solving inclusion problems and serves as the foundation for many numerical algorithms. Despite this popularity, its convergence results have been largely limited to the monotone setting. In this work, we study the convergence of (relaxed) preconditioned PPA for a class of nonmonotone problems that satisfy an oblique weak Minty condition. Additionally, we study the (relaxed) Douglas-Rachford splitting (DRS) method in the nonmonotone setting by establishing a connection between DRS and the preconditioned PPA with a positive semidefinite preconditioner. To better characterize the class of problems covered by our analysis, we introduce the class of semimonotone operators, offering a natural extension to (hypo)monotone and co(hypo)monotone operators, and describe some of their properties. Sufficient conditions for global convergence of DRS involving the sum of two semimonotone operators are provided. Notably, it is shown that DRS converges even when the sum of the involved operators (or of their inverses) is nonmonotone. Various example problems are provided, demonstrating the tightness of our convergence results and highlighting the wide range of applications our theory is able to cover.

==> TeX/Text/Examples/Intro/Nplayer.tex <==
%!TEX root = ../../../DRS-Minty.tex
\begin{example}{(N-player games)}
    More generally, we can consider arbitrary continuous games consisting of $N$ players. Let $x \coloneqq (x_i, x_{-i}) \coloneqq (x_1, \hdots, x_N)$ denote the decision variables, where $x_i$ represents the decision variables of the $i^{\textrm{th}}$ player, who is attempting to minimize his loss $\mathcal{L}_i(x_i, x_{-i})$. We are interested in finding a Nash equilibrium, which is a decision vector $x^*$ for which no player could improve his performance by unilaterally changing his decisions, i.e.,
    \begin{equation}
    \text{find}\quad x^\star \quad \text{such that} \quad \mathcal{L}(x_i^\star, x_{-i}^\star) \leq \mathcal{L}(x_i, x_{-i}^\star), \quad \forall x_i \text{ and } \forall i \in \{1, \hdots, N\}.\tag{P-3}
    \end{equation}
    The corresponding first order optimality conditions of this equilibrium problem may be written in the form of the structured inclusion~\eqref{prob:composite} by defining $\Tp x = (\partial_{x_1} \mathcal{L}_1(x), \hdots, \partial_{x_N} \mathcal{L}_N(x))$. The main question is how to properly decompose $\Tp$ into the sum of two operators $A$ and $B$ (with \(L = \id\)). Here, we will mainly focus on decompositions for which the resolvents can be computed in a distributed manner.

    First, consider a $2$\hyp{}player game. In this case, an obvious choice would be to select $Ax = (\partial_{x_1} \mathcal{L}_1(x), 0)$ and $Bx = (0, \partial_{x_2} \mathcal{L}_2(x))$, as this choice decomposes $\Tp$ into two player-specific terms. This results in a decentralized scheme, where the two resolvent computations in~\ref{eq:DRS} are solved in a successive manner by the respective players.

    For general $N$\hyp{}player games, a distributed scheme can be obtained by introducing additional variables. To this end, let each player extend its decision space to maintain its own local decision and a local estimate of other players' decision variables. Then, the loss of the each player can be decomposed as the sum of a player-specific loss term and a consensus term. The resulting DRS scheme then consists of player-specific resolvent computations, which can be evaluated in a distributed manner, and additional consensus steps. For more detailed information on this topic and on other decompositions for $N$\hyp{}player games, we refer the interested reader to \cite{huang2021Distributed,di2020Local,lecadre2022Parametrized}.
\end{example}

==> TeX/Text/Examples/Intro/minmax.tex <==
%!TEX root = ../../../DRS-Minty.tex
\begin{example}{(Min-max problems)}\label{example:minimax}
    % Examples are cited in https://arxiv.org/pdf/2110.04261.pdf
    % Recent applications in machine learning, such as robust reinforcement learning and the training of generative adversarial networks (GANs), have increased the importance of solving min-max optimization problems with nonconvex-nonconcave objectives, taking the following general form:
    To capture a wide range of applications in e.g. machine learning and control, we consider min-max optimization problems of the following general form:
    \begin{equation}\label{eq:example minimax problem}
        \minimize_{x_1\in\R^{n_1}} \maximize_{x_2\in\R^{n_2}} \mathcal{L}(x_1,x_2), \tagexampleproblem
    \end{equation}
    where $\mathcal{L} : \R^{n_1 \times n_2} \rightarrow \Rinf$.
    % is not necessarily convex in $x$ and/or concave in $y$.
    Traditionally, when applying Douglas-Rachford splitting to solve \eqref{eq:example minimax problem}, $\mathcal{L}(x,y)$ is assumed to be convex-concave and is decomposed into 
    $$
        \mathcal{L}(x_1,x_2) \coloneqq \psi_1(x_1,x_2) + \psi_2(x_1,x_2)
    $$
    where $\psi_1, \psi_2 : \R^{n_1 \times n_2} \rightarrow \Rinf$ are proper functions which are lower semicontinuous and convex in $x_1$ and upper semicontinuous and concave in $x_2$. The first order optimality condition associated with \eqref{eq:example minimax problem} may then be written in the form of the structured inclusion \eqref{prob:composite}
    by defining $Ax = (\partial_{x_1} \psi_1(x_1,y_2), -\partial_{x_2} \psi_1(x_1,x_2))$, $Bx = (\partial_{x_1} \psi_2(x_1,x_2), -\partial_{x_2} \psi_2(x_1,x_2))$, and \(L = \id\). 
    
    Since the main iterations in DRS are evaluations of the resolvents $J_{\gamma A} \coloneqq (\id + \gamma A)^{-1}$ and $J_{\gamma B} \coloneqq (\id + \gamma B)^{-1}$, usually $\psi_1$ and $\psi_2$ are chosen such that these resolvents are easy to compute. For example, one may choose $\psi_1$ to represent some (coupled) loss function while $\psi_2(x_1,y_2) \coloneqq g(x_1) - h(x_2)$ may represent regularization terms such as $\ell^1$ or $\ell^2$ norms, or indicator functions of sets allowing us to capture constrained minimax problems. In this case, since $g$ and $h$ are convex, the resolvent of $B$ is given by $J_{\gamma B}(x_1,x_2) = (\prox_{\gamma g}(x_1), \prox_{\gamma h}(x_2))$ \cite[Example 10.2]{rockafellar2009Variational}.
    
    In this work, we allow $\mathcal{L} : \R^{n_1 \times n_2} \rightarrow \Rinf$ to be not necessarily convex in $x_1$ and/or concave in $x_2$. As a result, we will only assume that $\psi_1, \psi_2$ are proper and lower semicontinuous, but possibly nonconvex-nonconcave. This allows Douglas-Rachford to be applied to a much larger range of applications, such as robust reinforcement learning and the training of generative adversarial networks.

    % If $A = \partial f$ is the subgradient of a proper function, then it is known that $\prox_{\gamma \partial f}(x) \subset (\id + \gamma \partial f)^{-1}(x)$, $\forall x$ \cite[Example 10.2]{rockafellar2009}. If $f$ is additionally lower semicontinuous and prox-bounded, then $\prox_{\gamma f}$ is nonempty- and compact-valued \cite[Thm. 1.25]{rockafellar2009}, such that the resolvent is full domain. 

    % Note that if $f$ is (hypo)convex, this inclusion holds as an equation
\end{example}

==> TeX/Text/Examples/Intro/optimization.tex <==
%!TEX root = ../../../DRS-Minty.tex
\begin{example}{(Optimization problems)}\label{example:sum of functions]}
    Many problems in optimization can be decomposed in the the minimization of the sum of two functions, i.e.
    \begin{equation}\label{eq:example sum of functions}
        \minimize_{x\in\R^n} \psi(x) = \psi_1(x) + \psi_2(x). \tagexampleproblem
    \end{equation}
    where $\psi_1, \psi_2$ are proper, lower semicontinuous (lsc) and extended-real-valued functions. The first order conditions of this optimization problem correspond to finding a zero of the sum of the subdifferential operators, i.e., solving the structured inclusion~\eqref{prob:composite} by defining \(L = \id\),  $A = \partial \psi_1$ and $B = \partial \psi_2$.
    
    If $\psi_1$ and $\psi_2$ are convex, then it is well known that $\partial \psi_1$ and $\partial \psi_2$ are maximally monotone \cite{minty1964monotonicity}. Furthermore, since the proximal mapping of a convex function corresponds to the resolvent of its subdifferential, the DRS iterations~\ref{eq:DRS} applied to~\eqref{eq:example sum of functions} can then be written equivalently as
    \begin{equation}
        \begin{cases}\tag{DRS-1}\label{eq:DRS_minimization}
            \displaystyle   
            \bar{x}^k &\in \prox_{\gamma \psi_1}(s^k)\\
            \hat{x}^k &\in \prox_{\gamma \psi_2}(2\bar{x}^k-s^k)\\
            s^{k+1} &= s^k + \lambda(\hat{x}^k - \bar{x}^k)
        \end{cases}
        \end{equation}
    and it can be easily seen that if $s$ is a fixed point of~\eqref{eq:DRS_minimization}, then $\bar{x} \in \prox_{\gamma \psi_1}(s)$ satisfies the first-order necessary condition. 
    % Furthermore, in the convex case, the DRS iterations are known to converge for any \gamma > 0$ and $\lambda \in (0, 2)$.
    % The first analysis of global convergence of iterations~\eqref{eq:DRS_minimization} in the nonconvex setting where one function is Lipschitz differentiable was provided in the work of Li and Pong \cite{li2016Douglas}, and later tightened in the work of Themelis and Patrinos \cite{themelis2020DouglasRachford}. 
    Note that in the nonconvex setting, iterations~\eqref{eq:DRS_minimization} are not exactly equivalent to~\ref{eq:DRS}, since the proximal mapping of a nonconvex function is only a subset of the resolvent of its subdifferential \cite[Example 10.2]{rockafellar2009Variational}.
\end{example}

==> TeX/Text/Examples/VonNeumannV.tex <==
As a second illustrative example, we will consider the application of our theory to the renowned mathematical-economic model of Von Neumann \cite{neumann1945model}, which was recently explored in \cite{daskalakis2020independent}.
\begin{example}[Von Neumann]\label{ex:VonNeumann}
    Using the standard definition of the simplex
    \(
    \Delta_d \coloneqq \set{x \in \R^d}[ x \geq 0, \sum_{i=1}^d x_i = 1]
    \),
    consider an economy where there are 
    $n$ goods with relative prices $v \in \Delta_n$,
    which can be produced by $m$ processes with relative intensities $u \in \Delta_m$.
    Let $R_{ij} \geq 0$ and $S_{ij} \geq 0$ denote the number of units of the $j$th good consumed and produced by the $i$th process, respectively. 
    % Assume that the total value of all goods produced is strictly positive, i.e., that $\inner{x, Sy} > 0$ for all $x \in \Delta_m$, $y \in \Delta_n$.
    By \cite[\S 5]{neumann1945model}, a pair $(u^\star, v^\star)$ for which this economy is expanding corresponds to a minimax solution of
    % there exist intensities $x^\star$ and prices $y^\star$ such that the economy is expanding if and only if there exists a saddle point solution to the minimax problem
    \begin{align*}
        \minimize_{u \in \Delta_m} 
        \;
        \maximize_{v \in \Delta_n} 
        \;
        f(u,v) \coloneqq \frac{\inner{u, Rv}}{{\inner{u, Sv}}}.
        \numberthis\label{eq:ex:neumann}
    \end{align*}
    % In other words, we need to find a zero of
    Defining $x \coloneqq (u, v)$, the problem of finding stationary points of \eqref{eq:ex:neumann} corresponds to finding a zero of
    $
        T(x) 
            {}\coloneqq{}
        F(x)
        +
        N_C(x)
    $,
    where
    $
        F(x)
            {}={}
        \begin{bsmallmatrix}
            \nabla_u f(u,v)^\top &
            - \nabla_v f(u,v)^\top
        \end{bsmallmatrix}^\top
        %     +
        % \begin{bsmallmatrix}
        %     N_{\Delta_m}(x)\\
        %     N_{\Delta_n}(y)
        % \end{bsmallmatrix}.
    $
    and 
    $
        C = \Delta_2 \times \Delta_2
    $.
    % Note that \eqref{eq:ex:neumann} can alternatively be interpreted as the value $f(u, v)$ for a stochastic game with a single state and mixed strategies \cite{daskalakis2020independent}.
\end{example}
In \cite[Prop. 2]{daskalakis2020independent}, it was observed numerically that for certain choices $R$ and $S$, operator $F$ is nonmonotone but satisfies the weak MVI.
In the following proposition, we formally show that the Nash equilibrium of \eqref{eq:ex:neumann} is a $\DRSRho$\hyp{}weak Minty solution of operator $T = F + N_C$. In this proposition, a scalar parameter $c$ is introduced to control the ratio between two different blocks in $\DRSRho$.
\ifspringer
    The proof can be found in the arXiv preprint \cite[Appendix C]{evens2023convergence} and a numerical experiment leveraging this result is provided in \Cref{fig:VonNeumann}.
\else
    The proof is deferred to \Cref{proof:prop:ex:neumann} and a numerical experiment leveraging this result is provided in \Cref{fig:VonNeumann}.
\fi
\begin{figure}
    \centering
    % \includetikz{Examples/VonNeumann/iterates_ppa}
	\includetikz{Examples/VonNeumann/iterates_pppa_combined}
    \caption{
        Visualization of the relaxed preconditioned proximal point algorithm with constant relaxation parameter $\lambda = \etamin$, applied to the ratio game from \Cref{ex:VonNeumann}.
        In this example, $\epsilon = \nicefrac15$, $R$ and $S$ are given by \eqref{eq:prop:ex:neumann:matrices} and $x \in \Delta_2 \times \Delta_2$ is parametrized by $x = (s, 1-s, t, 1-t)$.
        The unique Nash equilibrium is marked in green.
        % and its minimum value is given by $\DRSrho \approx -0.18$.
        By \Cref{prop:ex:neumann} with $c = 1$, the Nash equilibrium is a $\DRSrho$\hyp{}weak Minty solution of $T$ where $\DRSrho \approx -0.18$. 
        The colormap displays the value of the local weak Minty constant $\varrho\bigl(s, t, 1\bigr)$, as defined in \eqref{eq:prop:ex:neumann:localMinty}.
        (left) 
        Sequences generated using preconditioning matrix $\M_1 = 4\I_4$, for which $\etamin = \alpha_k = 1 + \lambda_{\rm min}(\DRSrho \M_1) \approx 0.29$.
        (right) Sequences generated using preconditioning matrix 
        $
            \M_2 = \blkdiag(\nicefrac83 \I_2, 8\I_2)
        $,
        for which $1 + \lambda_{\rm min}(\DRSrho \M_2) \approx -0.42$. Hence, under the regular weak Minty assumption, convergence of \ref{eq:PPPA-intro} can not be established for this preconditioner. 
        However. by \Cref{prop:ex:neumann} with $c = \nicefrac13$, the Nash equilibrium is also a $\DRSRho \approx \blkdiag(-0.27\I_2, -0.09\I_2)$\hyp{}oblique weak Minty solution of $T$,
        so that $\etamin = \alpha_k = 1 + \lambda_{\rm min}(\DRSRho \M_2) \approx 0.29$.
        % Therefore, \eqref{eq:PPPA-intro} converges under the larger class of problems with $\DRSRho$\hyp{}oblique weak Minty solutions.
    }
    \label{fig:VonNeumann}
\end{figure}

\begin{proposition}\label{prop:ex:neumann}
    Let $\epsilon \in (0,1)$ and let
    \begin{align*}
        R 
            {}={} 
        \begin{bmatrix}
            0 & 1 + \nicefrac{\epsilon}2\\
            2 - \nicefrac{\epsilon}2 & 2
        \end{bmatrix}
        \quad\text{and}\quad
        S
            {}={}
        \begin{bmatrix}
            \nicefrac12 & \nicefrac12\\
            1 & 1
        \end{bmatrix}.
        \numberthis\label{eq:prop:ex:neumann:matrices}
    \end{align*}
    % Let $\gamma, \kappa \in \R_{++}$ and consider the preconditioner $\M = \gamma^{-1} \blkdiag(\I_2, \kappa\I_2)$, which reduces to the classic preconditioner $\M = \gamma^{-1} \I_4$ when $\kappa = 1$.
    % Consider the stepsize parameters $\gamma_u, \gamma_v \in \R_{++}$ and the preconditioner $\M = \blkdiag(\gamma_u^{-1} \I_2, \gamma_v^{-1}\I_2)$.
    Let $c \in \R_+$ and $\tilde \DRSRho \coloneqq \blkdiag(\I_2, c\I_2)$.
    The unique Nash equilibrium 
    $
        x^\star \coloneqq (u^\star, v^\star) =
        \begin{bsmallmatrix}
            0 & 1 & 0 & 1
        \end{bsmallmatrix}^\top
    $
    of \eqref{eq:ex:neumann} is a $\DRSRho \coloneqq \DRSrho \tilde \DRSRho$\hyp{}oblique weak Minty solution of $T$, where $\rho$ is given by
    \begin{align*}
        \DRSrho 
            {}={}
        \inf_{
            (x, y) \in \graph N_C
            }
        \frac{
            \inner*{F(x) + y,x-x^\star}
        }
        {
            \qindef{F(x) + y}{\tilde \DRSRho}
        },
    \end{align*}
    which after parametrizing $x = (s, 1-s, t, 1-t)$ corresponds to the solution of 
    % the quasiconvex optimization problem
    \ifspringer
        \begin{align*}
            \DRSrho
                {}={}& 
            \min_{s, t}\; 
            \varrho(s, t, c)
                \coloneqq
            \tfrac{
                4(2 - s)^2
                (
                    \epsilon(s + t) - st(\epsilon + s)
                )
            }
            {
                (
                    2\epsilon - t(4 + \epsilon)
                )^2
                    +
                c
                (\epsilon + 2s)^2(2 - s)^2
            } \; \stt \;
            s \in (\sqrt{\epsilon}, 1],
            t \in \left(
                \tfrac{\epsilon s}{s(\epsilon + s)-\epsilon}, 1
            \right].
            \numberthis\label{eq:prop:ex:neumann:localMinty}
        \end{align*}
    \else
        \begin{align*}
            \DRSrho
                {}={}& 
            \min_{s, t}\; 
            \varrho(s, t, c)
                \coloneqq
            \frac{
                4(2 - s)^2
                (
                    \epsilon(s + t) - st(\epsilon + s)
                )
            }
            {
                (
                    2\epsilon - t(4 + \epsilon)
                )^2
                    +
                c
                (\epsilon + 2s)^2(2 - s)^2
            } \; \stt \;
            s \in (\sqrt{\epsilon}, 1],
            t \in \left(
                \frac{\epsilon s}{s(\epsilon + s)-\epsilon}, 1
            \right].
            \numberthis\label{eq:prop:ex:neumann:localMinty}
        \end{align*}
    \fi
\end{proposition}

==> TeX/Text/Examples/VonNeumann_tau.tex <==
\begin{proposition}
    Let $\epsilon, \tau \in (0,1)$ with $\epsilon < \tfrac{1-\tau}{2\tau}$. Let
    \begin{align*}
        R 
            {}={} 
        \begin{bmatrix}
            0 & 1 + \epsilon\\
            \tau^{-1} - \epsilon & \tau^{-1}
        \end{bmatrix}
        \quad\text{and}\quad
        S
            {}={}
        \begin{bmatrix}
            \tau & \tau\\
            1 & 1
        \end{bmatrix}.
    \end{align*}
    Then, the unique Nash equilibrium $
    z^\star = 
    \begin{bsmallmatrix}
        0 &1 &0 &1
    \end{bsmallmatrix}^\top
    $ is a $\DRSrho$-weak Minty solution of $T$, where 
    \begin{align*}
        \DRSrho 
            {}={}
        \minimize_{z \in \Delta_2 \times \Delta_2}
        \frac{2\inner{F(z), z - z^\star}}{\nrm{F_1(z) - F_2(z)}^2 + \nrm{F_3(z) - F_4(z)}^2}.
    \end{align*}
    \begin{proof}
        Observe that $f(x, y) - \tau^{-1} = \frac{\inner{x, \bar{R}y}}{{\inner{x, Sy}}}$ where 
        $
            \bar{R} 
                =
            \begin{bsmallmatrix}
                -1 & \epsilon\\
                - \epsilon & 0
            \end{bsmallmatrix}
        $.
        Consequently, if follows from \cite[Prop. 2]{daskalakis2020independent} that $z^\star$ is the unique Nash equilibrium of \eqref{eq:ex:neumann}.
        Using \cite[Ex. 5.2.6(c)]{Hiriart1996Convex}, observe that 
        \begin{align*}
            F(z)
                {}={}&
            \tfrac{1}{\inner{x, Sy}^2}
            \begin{bmatrix}
                \inner{x, Sy} Ry - \inner{x, Ry} Sy\\
                \inner{x, Ry} S^\top x - \inner{x, Sy} R^\top x
            \end{bmatrix}, \;
            N_C(z)
                {}={}
            \set{
                \alpha \otimes 
                \begin{bsmallmatrix}
                    1 \\ 1
                \end{bsmallmatrix}
                -
                \beta
            \,\middle|\, \alpha \in \R^2, \beta \in \R_+^4, \inner{\beta, z} = 0}.
        \end{align*}
        Therefore, to find the largest value of $\DRSrho$ we need to ensure that
        \begin{align*}
            \inner*{F(z) + v,z-z^\star} \geq \DRSrho \nrm*{F(z) + v}^2,\qquad \text{for all $(z,v)\in\graph N_C$}.
        \end{align*}
        Therefore,
        \begin{align*}
            \DRSrho 
                {}={}
            \minimize_{(z, v) \in \graph N_C} 
            \tfrac{
                \inner*{F(z) + v,z-z^\star}
            }
            {
                \nrm*{F(z) + v}^2
            }
                {}={}& 
            \minimize_{
                \substack{
                    % s,\, t \in [0,1],\\ 
                    z \in C,\\
                    \alpha \in \R^2,\, \beta \in \R_+^4
                }
            } \; \tfrac{
                \inner*{ 
                    F(z),
                    z - z^\star
                } 
                    +
                \inner*{                   
                    \alpha \otimes 
                    \begin{bsmallmatrix}
                        1 \\ 1
                    \end{bsmallmatrix}
                        -
                    \beta,
                    z - z^\star
                } 
            }
            {\nrm*{
                F(z)
                    +                         
                \alpha \otimes 
                \begin{bsmallmatrix}
                    1 \\ 1
                \end{bsmallmatrix}
                -
                \beta
            }^2
            }
            \; \stt \;
            \inner{
                \beta,
                z
            } 
            = 0
            \\
            {}={}& 
            \minimize_{
                \substack{
                    z \in C,\\ 
                    \alpha \in \R^2,\, \beta \in \R_+^4
                }
            } \; \tfrac{
                \inner*{ 
                    F(z),
                    z - z^\star
                } 
                    +
                \beta_2 z_2
                    +
                \beta_4 z_4
            }
            {\nrm*{
                F(z)
                    +                         
                \alpha \otimes 
                \begin{bsmallmatrix}
                    1 \\ 1
                \end{bsmallmatrix}
                -
                \beta
            }^2
            }
            \; \stt \;
            \inner{
                \beta,
                z
                } 
            = 0
        \end{align*}
        By \cite[Prop. 2]{daskalakis2020independent} there exist $z \in C$ so that 
        $
            \inner*{ 
                F(z),
                z - z^\star
            } < 0
        $.
        Consequently, $\alpha^\star$ minimizes the denominator, i.e.
        \begin{align*}
            % \alpha^\star(z, \beta)
            %     {}={}
            \minimize_{\alpha \in \R^2}\;
            \nrm*{
                F(z)
                    +                         
                \alpha \otimes 
                \begin{bsmallmatrix}
                    1 \\ 1
                \end{bsmallmatrix}
                -
                \beta
            }^2
                {}={}
            \tfrac12\bigl(F_1(z) - \beta_1 - F_2(z) + \beta_2\bigr)^2
                +
            \tfrac12\bigl(F_3(z) - \beta_3 - F_4(z) + \beta_4\bigr)^2
        \end{align*}
        and thus
        \begin{align*}
            \DRSrho 
                {}={}& 
            \minimize_{
                \substack{
                    z \in C,\\ 
                    \beta \in \R_+^4
                }
            } \; \tfrac{
                2\inner*{ 
                    F(z),
                    z - z^\star
                } 
                    +
                2\beta_2 s 
                    +
                2\beta_4 t
            }
            {
                \bigl(F_1(z) - \beta_1 - F_2(z) + \beta_2\bigr)^2
                    +
                \bigl(F_3(z) - \beta_3 - F_4(z) + \beta_4\bigr)^2
            }
            \; \stt \;
            \inner{
                \beta,
                z
                } 
            = 0
        \end{align*}
        Note that 
        $
            z \in C = \Delta_2 \times \Delta_2
        $
        can be parametrized as
        $
            z
                \coloneqq
            (s, 1-s, t, 1-t)
        $, so that
        \begin{align*}
            F(z)
                {}={}
            \tfrac{1}{(s\tau - s + 1)^2}
            \begin{bmatrix}
                \left(1 - s\right) \left(\epsilon t \tau - \epsilon t + \epsilon - t\right)\\
                - s \left(\epsilon t \tau - \epsilon t + \epsilon - t\right)\\
                \left(\epsilon + s - t \left(\epsilon + s\right)\right)\left(s \tau - s + 1\right)\\
                - t \left(\epsilon + s\right) \left(s \tau - s + 1\right)
            \end{bmatrix}
        \end{align*}
        and consequently 
        \begin{align*}
            \inner*{ 
                    F(z),
                    z - z^\star
                }
                {}={}&
            \tfrac{                        
                st(s + 2\epsilon)(\tau - 1) + \epsilon(s + t)
                }{(s\tau - s + 1)^2},
                \quad
            F_1(z) - F_2(z)
                {}={}
            \tfrac{\epsilon + t(\epsilon \tau - \epsilon - 1)}{(s\tau - s + 1)^2}, 
                \quad
            F_3(z) - F_4(z)
                {}={}
            \tfrac{\epsilon + s}{s\tau - s + 1}.
        \end{align*}
        Let $\bar{\beta} = (s\tau - s + 1)^2\beta$. Then, 
        \begin{align*}
            \DRSrho
                {}={}& 
            \minimize_{
                \substack{
                    s,t \in [0,1],\\ 
                    \bar{\beta} \in \R_+^4
                }
            } \;
            \tfrac{
                2(s\tau - s + 1)^2
                \bigl(
                    st(s + 2\epsilon)(\tau - 1) + \epsilon(s + t)
                        +
                    \bar{\beta}_2 s 
                        +
                    \bar{\beta}_4 t
                \bigr)
            }
            {
                \bigl(
                    \epsilon + t(\epsilon \tau - \epsilon - 1) 
                    + 
                    \bar{\beta}_2 - \bar{\beta}_1
                \bigr)^2
                    +
                \bigl(
                    (\epsilon + s)(s\tau - s + 1)
                    +
                    \bar{\beta}_4 - \bar{\beta}_3
                \bigr)^2
            }
            \; \stt \;
            \inner{
                \bar{\beta},
                % z
                \begin{bsmallmatrix}
                    s \\ 1-s \\ t \\ 1-t
                \end{bsmallmatrix}
                } 
            = 0
        \end{align*}
        Note that
        $
            \inner*{ 
                F(z),
                z - z^\star
            }
                <
            0
        $
        if and only if $s \in (\bar{s}, 1]$ and $t \in (\bar{t}(s), 1]$, where
        \begin{align*}
            \bar{s}
                {}\coloneqq{}
            \epsilon\sqrt{1+\nicefrac{1}{(1-\tau)\epsilon}} - \epsilon
            \quad\text{and}\quad
            \bar{t}(s)
                {}\coloneqq{}
            \tfrac{\epsilon s}{s(s+2\epsilon)(1-\tau)-\epsilon}.
        \end{align*}
        Consequently, 
        \begin{align*}
            \DRSrho
                {}={}& 
            \minimize_{
                \substack{
                    s \in (\bar{s}, 1],\\
                    t \in (\bar{t}(s), 1],\\ 
                    \bar{\beta}_2, \bar{\beta}_4 \in \R_+
                }
            } \; 
            \tfrac{
                2(s\tau - s + 1)^2
                \bigl(
                    st(s + 2\epsilon)(\tau - 1) + \epsilon(s + t)
                        +
                    \bar{\beta}_2 s 
                        +
                    \bar{\beta}_4 t
                \bigr)
            }
            {
                \bigl(
                    \epsilon + t(\epsilon \tau - \epsilon - 1) 
                    + 
                    \bar{\beta}_2
                \bigr)^2
                    +
                \bigl(
                    (\epsilon + s)(s\tau - s + 1)
                    +
                    \bar{\beta}_4
                \bigr)^2
            }
            \; \stt \;
            \inner{
                \begin{bsmallmatrix}
                    \bar{\beta}_2 \\ \bar{\beta}_4
                \end{bsmallmatrix},
                \begin{bsmallmatrix}
                    1-s \\ 1-t
                \end{bsmallmatrix}
                } 
            = 0
        \end{align*}
        Since $(\epsilon + s)(s\tau - s + 1) > 0$, it follows immediately that $\bar{\beta}_4^\star = 0$, so that
        \begin{align*}
            \DRSrho
                {}={}& 
            \minimize_{
                \substack{
                    s \in (\bar{s}, 1],\\
                    t \in (\bar{t}(s), 1],\\ 
                    \bar{\beta}_2 \in \R_+
                }
            } \; 
            \tfrac{
                2(s\tau - s + 1)^2
                \bigl(
                    st(s + 2\epsilon)(\tau - 1) + \epsilon(s + t)
                        +
                    \bar{\beta}_2 s
                \bigr)
            }
            {
                \bigl(
                    \epsilon + t(\epsilon \tau - \epsilon - 1) 
                    + 
                    \bar{\beta}_2
                \bigr)^2
                    +
                \bigl(
                    (\epsilon + s)(s\tau - s + 1)
                \bigr)^2
            }
            \; \stt \;
            \bar{\beta}_2(1-s) = 0
        \end{align*}
        First, consider the case where $s^\star \neq 1$. Then, we need to solve
        \begin{align*}
            \DRSrho
                {}={}& 
            \minimize_{
                \substack{
                    s \in (\bar{s}, 1],\\
                    t \in (\bar{t}(s), 1],\\ 
                    \bar{\beta}_2 \in \R_+
                }
            } \; 
            \tfrac{
                2(s\tau - s + 1)^2
                \bigl(
                    st(s + 2\epsilon)(\tau - 1) + \epsilon(s + t)
                        +
                    \bar{\beta}_2 s
                \bigr)
            }
            {
                \bigl(
                    \epsilon + t(\epsilon \tau - \epsilon - 1) 
                    + 
                    \bar{\beta}_2
                \bigr)^2
                    +
                \bigl(
                    (\epsilon + s)(s\tau - s + 1)
                \bigr)^2
            }
            \; \stt \;
            \bar{\beta}_2(1-s) = 0
        \end{align*}
        Owing the the constraint, it holds that $\bar{\beta}_2^\star = 0$ when $s^\star  \neq 1$. 
        Otherwise, let $a(t) \coloneqq \epsilon + t(\epsilon \tau - \epsilon - 1)$ and $b \coloneqq \tau (1 + \epsilon)$, so that 
        \begin{align*}
            \DRSrho
                {}={}& 
            \minimize_{
                \substack{
                    t \in (\bar{t}(1), 1],\\ 
                    \bar{\beta}_2 \in \R_+
                }
            } \; 
            g(t, \bar{\beta}_2)
                \coloneqq
            \tfrac{
                2\tau^2
                \bigl(
                    a(t) + b t
                        +
                    \bar{\beta}_2
                \bigr)
            }
            {
                \bigl(
                    a(t)
                    + 
                    \bar{\beta}_2
                \bigr)^2
                    +
                b^2
            }
        \end{align*}
        Using simple algebraic manipulation, it can be seen that for a fixed $t$, $g(t, \bar{\beta}_2)$ is decreasing if 
        \begin{align*}
            \bar{\beta}_2 < - a(t) - b(t + \sqrt{1 + t^2})
        \end{align*}
    \end{proof}
\end{proposition}

==> TeX/Text/Examples/toyV.tex <==
\begin{figure}
    \centering
    \includetikz{Examples/Ellipse/iterates}
    \caption{
        Visualization of the sequences $\seq{\bar x^k}$ for the 
                preconditioned proximal point algorithm
            with fixed relaxation parameter $\lambda$
        applied to \Cref{ex:pppa:ellipse}, where $a = 2$, $b = \nicefrac45$ and $c = \nicefrac54$
        and using preconditioner $\M = \diag(b, c)$%
        . 
        The zeros of $T$ are marked in green and its gradient flow $-T$ is indicated using gray arrows.
        (left) Sequences generated using $\lambda = 2.3 < \bar \lambda$, where $\bar \lambda$ is the upper bound on $\lambda_k$ from \eqref{eq:ex:pppa:ellipse:f2:lambda}. The orange sequence converges to the single $\bigl(\nicefrac{c}{a^2 + bc}, \nicefrac{b}{a^2 + bc}\bigr)$\hyp{}oblique weak Minty solution $(0,0)$ while the blue sequence converges to a zero of $T$ which is not a weak Minty solution (cf. \Cref{it:pppa:subseq}).
        (right) Sequences generated using $\lambda = 2.5 > \bar \lambda$. In this setting, it is no longer guaranteed by \Cref{thm:pppa} that the sequence $\seq{\bar x^k}$ converges, as can be seen from the (diverging) blue sequence.
        % Furthermore, the red sequence, for which $\lambda > 2.4$,  diverges. 
        % (right) 
        % The sequences 
        % \(
        %     \seq{\protect\min_{i=0, \dots, k} \nrm{\bar{v}^i}^2}
        % \) for the numerical experiments with $\lambda = 2.3$.
        % The thick lines represent the corresponding upper bounds on these sequences as given by \Cref{it:pppa:rate}. From this figure, it is apparent that these bounds are not tight in general.
        }
    \label{fig:ex:pppa:ellipse}
\end{figure}

\begin{example}[toy example]\label{ex:pppa:ellipse}
    \begin{minipage}[t]{0.195\textwidth}
        Consider the operator
        \begin{align*}
            \hspace{-3cm}
            T(x) \coloneqq f\Bigl(\nrm{\M x}\Bigr) 
            \begin{bmatrix}
                b & ab \\
                -ac & c
            \end{bmatrix}x,
        \end{align*}
    \end{minipage}%
    \begin{minipage}[t]{0.6\textwidth}
        % \begin{figure}
        \centering
        \vspace{-0.4cm}
        \includetikz{Examples/Ellipse/helper}
        \captionof{figure}{Definition of $f : \R_+ \rightarrow [0, 1]$ in \Cref{ex:pppa:ellipse}.}
        \label{fig:pppa:ellipse:f}
        % \end{figure}
    \end{minipage}

    \noindent
    where $a \in \R$, $b, c \in \R_{++}$, $\M \coloneqq \diag(1, \tfrac{c}{b})$ and $f : \R_+ \rightarrow [0, 1]$.
    If $f$ is defined as in \Cref{fig:pppa:ellipse:f}, then the following hold.
    \begin{enumerate}
        \item \label{it:ex:pppa:ellipse:f2:minty} 
        % If $\exists r \in \R_{++}: f(r) > 0$, then   
        $T$ has a single $\DRSRho = \bigl(\nicefrac{c}{a^2 + bc}, \nicefrac{b}{a^2 + bc}\bigr)$\hyp{}oblique weak Minty solution at the point $\pazocal{S}^\star = {(0,0)} \subset \zer T$ while the other zeros of $T$ are not $\DRSRho$\hyp{}oblique weak Minty solutions.
        \item \label{it:ex:pppa:ellipse:f2:convergence} 
        By \Cref{it:pppa:subseq}, the limit points of the sequence $\seq{\bar x^k}$ generated by the preconditioned proximal point algorithm with preconditioner $\M$ and fixed relaxation parameter $\lambda$ belong to $\zer T$ (not necessarily to $\pazocal{S}^\star$) if $\lambda$ lies in the interval
        \begin{align*}
            \begin{aligned}
                % \max_{i \in \{1,2\}} |\lambda_i(H)|^2
                % =\tfrac{\gamma^2a^2(\gamma b + (1-\lambda))^2 + (1 + \gamma b(1-\lambda))^2}{(1 + \gamma^2a^2)(1 + \gamma b)^2} < 1
                % \quad\Leftrightarrow\quad 
                0 < \lambda < \bar{\lambda} \coloneqq 2\left(1+\tfrac{bc}{a^2 + bc}\right).
            \end{aligned}\numberthis\label{eq:ex:pppa:ellipse:f2:lambda}
        \end{align*}
        This result has been verified numerically in \Cref{fig:ex:pppa:ellipse}.
    \end{enumerate}
    If $f \equiv 1$, then the following hold.
    \begin{enumerate}[resume]
        \item \label{it:ex:pppa:ellipse:f1:minty} 
        $T$ has a single $\DRSRho = \bigl(\nicefrac{c}{a^2 + bc}, \nicefrac{b}{a^2 + bc}\bigr)$\hyp{}oblique weak Minty solution at $\pazocal{S}^\star = \zer T = {(0,0)}$. 
        \item \label{it:ex:pppa:ellipse:f1:convergence} 
        By \Cref{it:pppa:full}, the sequence $\seq{\bar x^k}$ generated by the proximal point algorithm with fixed relaxation parameter $\lambda$ converges to $\zer T$ if $\lambda$ is selected according to \eqref{eq:ex:pppa:ellipse:f2:lambda}.
        By examining the spectral radius of the algorithmic operator, it can be seen that this result is tight.
    \end{enumerate}
    \begin{proof}
        Recall that for a given $\DRSRho \in \sym{2}$, the $\DRSRho$\hyp{}oblique weak Minty solutions of this problem are given by the set $\pazocal{S}^\star \subseteq \zer T$ for which it holds that
        \begin{align*}
            \inner{T(x), x - x^\star} \geq \qindef{T(x)}{\DRSRho},\quad \forall x \in \R^2, x^\star\in\pazocal{S}^\star.
            \numberthis\label{eq:ex:pppa:ellipse:WMVI}
        \end{align*}
        % \begin{itemize}
        %     \item test
        % \end{itemize}
        % \vspace{-0.6cm}
        \vspace{-\baselineskip}
        \begin{proofitemize}
            \item \ref{it:ex:pppa:ellipse:f2:minty} : The analytical expression for $f$ as defined in \Cref{fig:pppa:ellipse:f} is given by
            \begin{align*}
                f\Bigl(\nrm{\M x}\Bigr) \coloneqq 
                \begin{cases}
                    \nrm{x}_\M, & \quad \text{if } \nrm{\M x} \leq \nicefrac25,\\
                    \nicefrac45-\nrm{\M x}, & \quad \text{if }\nrm{\M x} \in \bigl(\nicefrac25, \nicefrac45\bigr),\\
                    0, & \quad \text{if } \nrm{\M x} \in \bigl[\nicefrac45, 1\bigr],\\
                    \nicefrac52\bigl(\nrm{\M x} - 1\bigr), & \quad \text{if } \nrm{\M x} \in \bigl(1, \nicefrac75\bigr),\\1, &\quad \text{if } \nrm{\M x} \geq \nicefrac75.
                \end{cases}
            \end{align*}
            Therefore, by definition of $T$, it holds that
            $\zer T = \set{x \in \R^2}[\nrm{x}_\M \in \{0\} \cup{[\nicefrac45, 1]}]$.
            Let 
            $
                \DRSRho 
                    \coloneqq
                \diag(\rho, \tfrac{b}{c}\rho)
            $
            for some $\rho \in \R$.
            Then, \eqref{eq:ex:pppa:ellipse:WMVI} corresponds to
            \begin{align*}
                f\Bigl(\nrm{x}_\M\Bigr)\Bigl(\nrm{x}_\M^2 - \bigl(b x_1 x_1^\star + c x_2 x_2^\star\bigr) + a\bigl(bx_1x_2^\star - cx_1^\star x_2\bigr)\Bigr) 
                    {}\geq{}
                \rho\tfrac{a^2 + bc}{c} f\Bigl(\nrm{x}_\M\Bigr)^2 \nrm{x}_\M^2,
                \qquad \forall x \in \R^2, x^\star\in\pazocal{S}^\star.
                \numberthis\label{eq:ex:pppa:ellipse:WMVI:T}
            \end{align*}
            This obviously holds for all $x \in \zer T$. For $x \notin \zer T$, we distinguish between the following two cases.
            % Let $x \notin \zer T$. Then, this holds iff 
            % \begin{align*}
            %     b + \tfrac{a(x_1x_2^\star - x_1^\star x_2) - b(x_1 x_1^\star + x_2 x_2^\star)}{\nrm{x}^2}
            %         {}\geq{}
            %     \rho (a^2 + b^2) f\bigl(\nrm{x}\bigr).
            % \end{align*}
            \begin{proofitemize}
                \item $\nrm{x^\star} = 0$: Then, \eqref{eq:ex:pppa:ellipse:WMVI:T} holds iff for all $x \notin \zer T$ it holds that
                \(
                    \rho
                        {}\leq{}
                    \tfrac{c}{(a^2 + bc) f\left(\nrm{x}_\M\right)}.
                    %     {}\leq{}
                    % \tfrac{b}{a^2 + b^2}.
                \)
                Since $f\left(\nrm{x}_\M\right) \in (0,1]$, this condition is satisfied for
                \(
                    \rho = \nicefrac{c}{a^2 + bc}.
                \)
                \item $\nrm{x^\star} \in [\nicefrac45, 1]$: Let $x = \epsilon x^\star$ where $\epsilon \in (0,\nicefrac25)$. Then, 
                % $x \notin \zer T$, 
                $f(\nrm{x}_\M) = \epsilon\nrm{x^\star}_\M$ and \eqref{eq:ex:pppa:ellipse:WMVI:T} holds iff
                \(
                    \rho 
                        {}\leq{}
                    \tfrac{
                        c(1 - \epsilon^{-1})
                    }{                    
                        \epsilon(a^2 + bc) \nrm{x^\star}_\M
                    }
                \)
                Taking the limit for $\epsilon$ to zero from above, we get that 
                $
                    \lim_{\epsilon \rightarrow 0+} 
                    \tfrac{c(1 - \epsilon^{-1})}{\epsilon(a^2 + bc) \nrm{x^\star}_\M}
                        {}={}
                    - \infty
                $
                and thus \eqref{eq:ex:pppa:ellipse:WMVI:T} can not be satisfied for any $\rho \in \R$.
            \end{proofitemize}
            \item \ref{it:ex:pppa:ellipse:f1:minty}: By definition of $T$ and using that $f \equiv 1$, it is straightforward to verify that $\zer T = {(0,0)}$ and that
            \eqref{eq:ex:pppa:ellipse:WMVI} holds for $\DRSRho = \bigl(\nicefrac{c}{a^2 + bc}, \nicefrac{b}{a^2 + bc}\bigr)$.
            \item \ref{it:ex:pppa:ellipse:f1:convergence}: 
            To show that the result from \Cref{it:pppa:full} is tight, define
            \begin{align*}
                H 
                    {}\coloneqq{}&
                \I_2 + \lambda\left((\M + T)^{-1}\M-\I_2\right)
                    {}={}
                \I_2 + \lambda\left(
                    \begin{bmatrix}
                        2b & a \\
                        -a & 2c
                    \end{bmatrix}^{-1}
                    \begin{bmatrix}
                        b & 0 \\
                        0 & c
                    \end{bmatrix}-\I_2\right)
                    {}={}
                % \I_2 + \lambda\left(
                %     \tfrac{1}{4bc+a^2}
                %     \begin{bmatrix}
                %         2c & -a \\
                %         a & 2b
                %     \end{bmatrix}
                %     \begin{bmatrix}
                %         b & 0 \\
                %         0 & c
                %     \end{bmatrix}-\I_2\right)
                %     {}={}
                \I_2 + \lambda\left(
                    \tfrac{1}{4bc+a^2}
                    \begin{bmatrix}
                        2bc & -ac \\
                        ab & 2bc
                    \end{bmatrix} -\I_2\right),
            \end{align*}
            such that the iteration of the proximal point algorithm with fixed relaxation parameter $\lambda$ can be expressed as the linear dynamical system $x^{k+1} = H x^k$. This system is globally asymptotically stable if and only if the spectral radius of \(H\) is strictly less than one, which through elementary algebra can be shown to hold iff \eqref{eq:ex:pppa:ellipse:f2:lambda} is satisfied, completing the proof.
            \qedhere
        \end{proofitemize}
    \end{proof}
\end{example}

==> TeX/Text/ProblemFormulation/DRS.tex <==
%!TEX root = ../../../DRS-Minty.tex

The classical DRS algorithm \cite{douglas1956Numerical} is applicable to inclusion \eqref{prob:composite}. 
Given stepsize $\gamma > 0$ and relaxation parameters $\lambda_k > 0$, and with initial point $s^0\in\R^n$, DRS consists of the following iterates.
\begin{equation}
\begin{cases}\tag{DRS}\label{eq:DRS}
    \displaystyle   
    \bar{x}^k&\in J_{\gamma \A}(s^k)\\
    \hat{x}^k&\in J_{\gamma \B}(2\bar{x}^k-s^k)\\
    s^{k+1}&=s^k+\lambda_k(\hat{x}^k-\bar{x}^k).
\end{cases}
\end{equation}
% where $J_{\gamma \A}$ and $J_{\gamma \B}$ denote the resolvents of $\gamma A$ and $\gamma B$. 
Despite the fact that \ref{eq:DRS} is a primal algorithm, our convergence analysis for \ref{eq:DRS} will rely on interpreting it as \ref{eq:PPPA-intro} applied to the primal-dual operator \eqref{eq:primaldual}, with preconditioning 
\begin{align}
    \M
        {}={}
    \begin{bmatrix}
        \gamma^{-1}\I_n&-\I_n\\
        -\I_n&\gamma \I_n
    \end{bmatrix}.
    \label{eq:M}
\end{align}
% In fact, letting \(z^k =(x^k,y^k)\), \(\bar z^k =(\bar x^k, \bar y^k)\), the iterates of PPA were already shown to lead to \eqref{eq:CP:alg:inclusion}. 
Defining \(s^k \coloneqq x^k - \gamma y^k\) and \(\hat x^k \coloneqq 2 \bar x^k - s^k - \gamma \bar y^k\), and using~\cite[Lemma 12.14, Example 12.13]{rockafellar2009Variational}, a generalization of Moreau's decomposition, leads to the elimination of the dual sequence \(\seq{y^k}\) and leads to \ref{eq:DRS}.


==> TeX/Text/ProblemFormulation/PrimalDual.tex <==
%!TEX root = ../../../DRS-Minty.tex
A prominent special case of \eqref{prob:P1} is to study problems where \(T\) (in this framework denoted \(\Tp\)) is decomposed as
\begin{equation}\label{prob:composite}\tag{P-I}
     0 \in \Tp x \coloneqq Ax + B x, 
\end{equation}
where $A : \R^n \rightrightarrows \R^n$, $B : \R^m \rightrightarrows \R^m$ are two (possibly nonmonotone) operators.  

For example, in the framework of convex optimization, \(A\) and \(B\) represent subdifferentials of proper lsc convex functions \(g\), \(h\), and inclusion \eqref{prob:composite} corresponds to the first-order optimality conditions of 
\[
    \minimize_{x\in\R^n} \; g(x) + h(x).
\]
The associated dual problem is to find a minimizer of \(g^*(-y) + h^*(y)\). Under standard constraint qualifications the set of solutions for the dual problem is nonempty and the duality gap is zero \cite[Cor. 31.2.1]{Rockafellar1970Convex}. 

However, duality theory is not limited to the monotone setting. In what follows, we set up the abstract duality framework introduced in \cite{attouch1996general}, \cite[Section 6.9]{auslender2006Asymptotic}. 
Problem \eqref{prob:composite} will be referred to as the primal inclusion.

Associated with the primal inclusion is the dual inclusion, given by
\begin{equation}\label{eq:dual}\tag{D-I}
    0\in \Td y 
    {}\coloneqq{}
    -A^{-1}(-y)+B^{-1}(y).
\end{equation}
A key property of the dual inclusion is that the primal inclusion is solvable if and only if the dual inclusion is solvable \cite[Proposition 6.9.1]{auslender2006Asymptotic}.
Additionally, we introduce the primal-dual inclusion associated with \eqref{prob:composite}, given by
\begin{equation}\label{eq:primaldual}\tag{PD-I}
\begin{bmatrix}0\\ 0\end{bmatrix}\in \overbracket*{\begin{bmatrix}Ax\\ B^{-1}y\end{bmatrix}+\begin{bmatrix}y\\ -x\end{bmatrix}}^{\Tpd z}.
\end{equation}
For this primal-dual inclusion, it holds that \cite[Proposition 6.9.2]{auslender2006Asymptotic}
$$
\begin{aligned}
    (x^\star,y^\star) &\in\zer \Tpd \iff (x^\star,- y^\star)\in\graph A,\ (x^\star,y^\star)\in\graph B,
\end{aligned}
$$
where \(\zer\Tp = \{x^\star \mid \exists y^\star : (x^\star,y^\star) \in\zer \Tpd\}\) and \(\zer\Td = \{y^\star \mid \exists x^\star : (x^\star,y^\star) \in\zer \Tpd\}\).

Furthermore, $(x^\star,y^\star)$ is a solution of the primal dual inclusion if and only if $x^\star$ is a solution of the primal inclusion and $y^\star$ is a solution of the dual inclusion.


==> TeX/Text/ProblemFormulation/ProbForm.tex <==
%!TEX root = ../../../DRS-Minty.tex
In this section, we will first briefly introduce the preconditioned proximal 
point algorithm.
Subsequently, the Chambolle-Pock splitting algorithm will be introduced and it
will be shown that CP is equivalent to the preconditioned proximal point 
algorithm applied to the primal-dual operator.
Finally, we will show that the Douglas--Rachford splitting algorithm is a 
specific instance of CP, and relate it to the preconditioned proximal point 
algorithm as well.
The convergence conditions for different algorithms and the corresponding proofs will be deferred to their respective sections later in the paper.



==> TeX/Text/Proofs/Additional/matrix.tex <==
%!TEX root = ../../../DRS-Minty.tex

\begin{definition}[Similarity] 
    \cite[Def. 1.3.1]{horn2012matrix}
    Let $A, B \in \R^{n \times n}$. $A$ is said to be similar to $B$ if there exists a nonsingular matrix $S \in \R^{n \times n}$ such that
    \[
        B = S^{-1} A S.
    \]
    The transformation $A \rightarrow S^{-1} A S$ is called a similarity transformation by the similarity matrix $S$. 
\end{definition}

\begin{proposition}
    \cite[Cor. 1.3.4]{horn2012matrix}
    If $A$ is similar to $B$, then $A$ and $B$ have the same eigenvalues.
\end{proposition}

==> TeX/Text/Proofs/Comonotone/resolvent_full.tex <==
%!TEX root = ../../../../DRS-Minty.tex

\begin{proposition}[resolvent of a comonotone operator]\label{prop:comon:fulldom}
    Let $T: \R^n \rightrightarrows \R^n$ be a $\DRSRho$\hyp{}comonotone operator and suppose that \(\M\) is selected according to \Cref{ass:PPPA:2}.
    Then, the following hold.
    \begin{enumerate}
        \item \label{prop:comon:resolvent} The preconditioned resolvent \(\PRES\) has full domain if and only if \(T\) is maximal.  
        \item \label{prop:comon:Lip} If \(\M \succ 0\), the preconditioned resolvent \(\PRES\) is Lipschitz continuous with Lipschitz constant
        \[
            L(\M) = \tfrac{\nrm{\M + \M\DRSRho\M} + \sqrt{\nrm{\M + \M\DRSRho\M}^2 - 4\lambda_{\rm min}(\M + \M\DRSRho\M)\lambda_{\rm min}(\M\DRSRho\M)}}{2\lambda_{\rm min}(\M + \M\DRSRho\M)}.
        \]
    \end{enumerate}
    \begin{proof}
        \begin{proofitemize}
            \item \ref{prop:comon:resolvent}:
            Since $T$ is $\DRSRho$\hyp{}comonotone, it holds by definition that 
            \(
                T^{-1} - \DRSRho 
            \)
            is monotone and thus also that
            \(
                \tilde T \coloneqq 
                % U^\top (T^{-1} - \DRSRho) U
                U^\top T^{-1} U - U^\top \DRSRho U
            \)
            is monotone.
            Furthermore, it holds that \((U^\top \M U)^{-1} + U^\top \DRSRho U \succ 0\) by \Cref{ass:PPPA:2,rem:ass:PPPA:eigcond}.
            Denote 
            \(
                \hat T \coloneqq U^\top T^{-1} U + (U^\top \M U)^{-1}
            \). 
            % First, we will show that \(\omega + \tfrac{1}{\theta} > 0\)  
            Owing to \((U^\top \M U)^{-1} + U^\top \DRSRho U \succ 0\) and Minty's theorem \cite[Thm. 21.1]{bauschke2017Convex}, the operator 
            \[
                \bigl((U^\top \M U)^{-1} + U^\top \DRSRho U\bigr)^{-1}\hat T 
                    {}={}
                \bigl((U^\top \M U)^{-1} + U^\top \DRSRho U\bigr)^{-1}\tilde T
                    {}+{}
                \id
            \]
            has full range iff \(\bigl((U^\top \M U)^{-1} + U^\top \DRSRho U\bigr)^{-1}\tilde T\) is maximally monotone.
            Since \((U^\top \M U)^{-1} + U^\top \DRSRho U \succ 0\), this implies that \(\hat T\) has full range iff \(\tilde T\) is maximally monotone, i.e., iff \(T\) is maximally $\DRSRho$\hyp{}comonotone.
    
            Therefore, it only remains to show that \(\hat T\) has full range iff 
            % \(\range{\M} \subseteq \range{\M+T}\),
            \(\dom{\PRES} = \R^n\).
            First suppose that \(\hat T\) has full range.
            Let $m$ denote the dimension of the range of \(\M\) and fix \(\hat{y}\in\R^m\).
            Then, by the full range assumption for \(\hat T\), there exists some \(\hat{x}\in\R^m\) such that \(\hat{y} \in \hat{T} \hat{x}\). 
            Letting \(\hat{z} = \hat{y} - (U^\top \M U)^{-1} \hat{x}\), this implies that 
            \begin{align*}
                \hat{y} \in U^\top T^{-1} U \hat{x} + (U^\top \M U)^{-1} \hat{x}
                    {}\iff{}
                \hat{z} \in U^\top T^{-1} U \bigl(U^\top \M U (\hat{y} - \hat{z})\bigr)
                \numberthis\label{eq:prop:comon:fulldom:equiv:1}
            \end{align*}
            Multiplying by $U$, this implies that \(U \hat{z} \in \projQ T^{-1} \bigl(\M U (\hat{y} - \hat{z})\bigr)\).
            Defining \(x' = U \hat{x}\), \(y' = U \hat{y}\) and \(z' = U \hat{z}\), this corresponds to 
            \(
                z' \in \projQ T^{-1} \bigl(\M (y' - z')\bigr).
            \)
            Consequently, \(T^{-1} \bigl(\M (y' - z')\bigr)\) is nonempty and there exists a $z'' \in \ker{\M} \subseteq \R^n$ so that
            \(
                z'' \in \proj_{\ker{\M}} T^{-1} \bigl(\M (y' - z')\bigr).
            \)
            Summing both inclusions, it holds that
            \begin{align*}
                z' + z'' \in T^{-1} \bigl(\M (y' - z')\bigr)
                    {}\iff{}
                \M (y' - z') \in T (z' + z'')
                %     {}\iff{}
                % \M y' \in \big(\M + T\big) (z' + z'')
                    {}\iff{}
                z' + z'' \in \big(\M + T\big)^{-1} \M y'
                %     {}\iff{}
                % z \in \big(\M + T\big)^{-1} \M y.
                \numberthis\label{eq:prop:comon:fulldom:equiv:2}
            \end{align*}
            % where $z \coloneqq z' + z''$ and $y \coloneqq y' + y''$.
            Since the choice of \(y'\) is arbitrary in \(\range{\M}\), \(\bigl(\M + T\bigr)^{-1} \M\) has full domain. 
    
            The converse follows similarly.
            Assume that \(\dom{\bigl(\M + T\bigr)^{-1} \M}=\R^n\).
            Then, for any fixed \(\hat{y}\in\R^m\) and \(y' = U \hat{y}\) there exists some \(z\in\R^n\) such that \(z \in (T + \M)^{-1}\M y\).
            Without loss of generality, decompose \(z \coloneqq U \hat{z} + z''\), where $z \in \R^m$ and \(z'' \in \ker{P}\). Then, by \eqref{eq:prop:comon:fulldom:equiv:2} it follows that
            \(
                U \hat{z} + z'' \in T^{-1} \bigl(\M U (\hat{y} - \hat{z})\bigr)
            \).
            Multiplying by $U^\top$, this implies that
            \(
                \hat{z} \in U^\top T^{-1} U \bigl(U^\top \M U (\hat{y} - \hat{z})\bigr)
            \).
            Defining $\hat{x} = U^\top P U (\hat{y} - \hat{z})$ and using \eqref{eq:prop:comon:fulldom:equiv:1}, we obtain \(\hat{y}\in \hat{T}\hat{x}\),  thus establishing that \(\hat T\) has full range.
            \item \ref{prop:comon:Lip}: 
            Take $(u,v), (\other{u}, \other{v}) \in \gph (\M + T)^{-1}\M$. By comonotonicity of \(T\) and using the fact that  
            \(
                \M(u-v) \in Tv,
            \) 
            \(
                \M(\other{u}-\other{v}) \in T\other{v}
            \),
            we have 
            \begin{align*}
                \qindef{(u-v)-(\other{u}-\other{v})}{\M\DRSRho\M}
                \leq
                \inner{\M \Bigl((u-v)-(\other{u}-\other{v})\Bigr), v-\other{v}}.
            \end{align*}
            Expanding the last term of the left-hand side and rearranging, we get
            \begin{align*}
                \qindef{u - \other{u}}{\M\DRSRho\M}
                +
                \qindef{v - \other{v}}{\M + \M\DRSRho\M}
                    {}\leq{}&
                \inner{(\M + 2\M\DRSRho\M) (u-\other{u}), v-\other{v}},
                %     {}\leq{}&
                % \nrm{\M + 2\M\DRSRho\M}\nrm{u-\other{u}}\nrm{v-\other{v}}.
            \end{align*}
            which implies that
            \begin{align*}
                \lambda_{\rm min}(\M \DRSRho \M)\nrm{u - \other{u}}^2
                +
                \lambda_{\rm min}(\M + \M\DRSRho\M)\nrm{v - \other{v}}^2
                    {}\leq{}&
                \nrm{\M + 2\M\DRSRho\M}\nrm{u-\other{u}}\nrm{v-\other{v}}
            \end{align*}
            If $\M \succ 0$, it holds that 
            \(\M + \M \DRSRho \M \succ 0\)
            by \Cref{ass:PPPA:2,rem:ass:PPPA:eigcond}.
            Hence, if \(u=\other{u}\) then necessarily \(v=\other{v}\), and the Lipschitz inequality holds trivially. 
            Otherwise, divide both sides by \(\|u-\other{u}\|^2\) to obtain 
            \begin{equation*}
                    \lambda_{\rm min}(\M + \M\DRSRho\M)\omega^2
                        - 
                    \nrm{\M + 2\M\DRSRho\M} \omega 
                        +
                    \lambda_{\rm min}(\M \DRSRho \M)
                        \leq 0,
            \end{equation*}
            where     
            \(
                \omega \coloneqq \tfrac{\nrm{v-\other{v}}}{\nrm{u-\other{u}}}    
            \). 
            Solving this quadratic inequality for $\omega$ yields the claimed Lipschitz modulus.
          \end{proofitemize}
    \end{proof}
\end{proposition}

==> TeX/Text/Proofs/Examples/VonNeumannV.tex <==

\begin{appendixproof}{prop:ex:neumann}[(Von Neumann)]
    Observe that $f(u, v) - 2 = \frac{\inner{u, \bar{R}v}}{{\inner{u, Sv}}}$ where 
    $
        \bar{R} 
            =
        \begin{bsmallmatrix}
            -1 & \nicefrac{\epsilon}{2}\\
            - \nicefrac{\epsilon}{2} & 0
        \end{bsmallmatrix}
    $.
    Consequently, if follows from \cite[Prop. 2]{daskalakis2020independent} that $x^\star$ is the unique Nash equilibrium of \eqref{eq:ex:neumann}.
    Using \cite[Ex. 5.2.6(c)]{Hiriart1996Convex} and recalling that $C \coloneqq \Delta_2 \times \Delta_2$, observe that 
    \begin{align*}
        F(x)
            {}={}&
        \begin{bmatrix}
            F_1(x) \\ F_2(x) \\ F_3(x) \\ F_4(x)
        \end{bmatrix}
            {}={}
        \tfrac{1}{\inner{u, Sv}^2}
        \begin{bmatrix}
            \inner{u, Sv} Rv - \inner{u, Rv} Sv\\
            \inner{u, Rv} S^\top u - \inner{u, Sv} R^\top u
        \end{bmatrix}, \;
        N_C(x)
            {}={}
        % N_{\Delta_2 \times \Delta_2}(x)
        %     {}={}
        \set{
            \alpha \otimes 
            \begin{bsmallmatrix}
                1 \\ 1
            \end{bsmallmatrix}
            -
            \beta
        \,\middle|\, \alpha \in \R^2, \beta \in \R_+^4, \inner{\beta, x} = 0}.
    \end{align*}
    Consequently, 
    \begin{align*}
        \DRSrho 
            {}={}
        \inf_{(x, y) \in \gph N_C}
        \tfrac{
            \inner*{F(x) + y,x-x^\star}
        }
        {
            \qindef{F(x) + y}{\tilde \DRSRho}
        }
            {}={}& 
        \inf_{
            \substack{
                % s,\, t \in [0,1],\\ 
                x \in C,\\
                \alpha \in \R^2,\, \beta \in \R_+^4
            }
        } \; \tfrac{
            \inner*{ 
                F(x),
                x - x^\star
            } 
                +
            \inner*{                   
                \alpha \otimes 
                \begin{bsmallmatrix}
                    1 \\ 1
                \end{bsmallmatrix}
                    -
                \beta,
                x - x^\star
            } 
        }
        {\qindef{
            F(x)
                +                         
            \alpha \otimes 
            \begin{bsmallmatrix}
                1 \\ 1
            \end{bsmallmatrix}
            -
            \beta
        }{\tilde \DRSRho}
        }
        \; \stt \;
        \inner{
            \beta,
            x
        } 
        = 0.
    \end{align*}
    Consider the parametrization 
    $
        x
            \coloneqq
        (s, 1-s, t, 1-t)
        % \begin{bsmallmatrix}
        %     s & 1-s & t & 1-t
        % \end{bsmallmatrix}^\top
    $
    where $s, t \in [0,1]$. Since     
    $
        x^\star =
        \begin{bsmallmatrix}
            0 & 1 & 0 & 1
        \end{bsmallmatrix}^\top
    $,
    it follows that
    \begin{align*}
        \inner*{                   
                \alpha \otimes 
                \begin{bsmallmatrix}
                    1 \\ 1
                \end{bsmallmatrix},
                x - x^\star
            }
            {}={}
        \inner*{                   
            \begin{bsmallmatrix}
                \alpha_1 \\ \alpha_1 \\ \alpha_2 \\ \alpha_2
            \end{bsmallmatrix},
            \begin{bsmallmatrix}
                s \\ -s \\ t \\ -t
            \end{bsmallmatrix}
            }
            {}={}
        0.
    \end{align*}
    Combining this with $\inner{\beta, x} = 0$ and $\inner{\beta, x^\star} = \beta_2 + \beta_4$, we get that
    \begin{align*}
        \DRSrho
            {}={}& 
        \inf_{
            \substack{
                x \in C,\\ 
                \alpha \in \R^2,\, \beta \in \R_+^4
            }
        } \; \tfrac{
            \inner*{ 
                F(x),
                x - x^\star
            } 
                +
            \beta_2
                +
            \beta_4
        }
        {\qindef{
            F(x)
                +                         
            \alpha \otimes 
            \begin{bsmallmatrix}
                1 \\ 1
            \end{bsmallmatrix}
            -
            \beta
        }{\tilde \DRSRho}
        }
        \; \stt \;
        \inner{
            \beta,
            x
            } 
        = 0.
    \end{align*}
    By \cite[Prop. 2]{daskalakis2020independent} there exist $x \in C$ so that 
    $
        \inner*{ 
            F(x),
            x - x^\star
        } < 0
    $, and thus by construction $\rho < 0$.
    Consequently, the numerator is negative at the infimum (take e.g. $\beta_2 = \beta_4 = 0$) and as such $\alpha$ minimizes the denominator at the infimum.
    Using that
    \begin{align*}
        \argmin_{\alpha \in \R^2} \;
        \qindef{
            F(x)
                +                         
            \alpha \otimes 
            \begin{bsmallmatrix}
                1 \\ 1
            \end{bsmallmatrix}
            -
            \beta
        }{\tilde \DRSRho}
            {}={}
        \tfrac12
        \begin{bmatrix}
            F_1(x) - F_2(x) - \beta_1 + \beta_2\\ 
            F_3(x) - F_4(x) - \beta_3 + \beta_4
        \end{bmatrix}
    \end{align*}
    this implies that
    \begin{align*}
        \DRSrho 
            {}={}& 
        \inf_{
            \substack{
                x \in C,\\ 
                \beta \in \R_+^4
            }
        } \; \tfrac{
            2\inner*{ 
                F(x),
                x - x^\star
            } 
                +
            2\beta_2
                +
            2\beta_4
        }
        {
            \bigl(
                F_1(x) - \beta_1 - F_2(x) + \beta_2
            \bigr)^2
                +
            c
            \bigl(
                F_3(x) - \beta_3 - F_4(x) + \beta_4
            \bigr)^2
        }
        \; \stt \;
        \inner{
            \beta,
            x
            } 
        = 0.
        \numberthis\label{eq:ex:Neumann:rho:1}
    \end{align*}
    Using aforementioned parametrization of $x$, it holds that
    % \begin{align*}
    %     F(x)
    %         {}={}
    %     \tfrac{1}{(1 - \nicefrac{s}{2})^2}
    %     \begin{bmatrix}
    %         \left(1 - s\right) \left(\epsilon - t(1 + \nicefrac{\epsilon}2)\right)\\
    %         - s \left(\epsilon - t(1 + \nicefrac{\epsilon}2)\right)\\
    %         \left(\epsilon + s - t \left(\epsilon + s\right)\right)(1 - \nicefrac{s}{2})\\
    %         - t \left(\epsilon + s\right) (1 - \nicefrac{s}{2})
    %     \end{bmatrix}
    % \end{align*}
    % and consequently 
    \begin{align*}
        \inner*{ 
                F(x),
                x - x^\star
            }
            {}={}&
        \tfrac{                        
                \epsilon(s + t)
                -
                st(\epsilon + s)
            }{
                \nicefrac12(2 - s)^2
            },
            \quad
        F_1(x) - F_2(x)
            {}={}
        \tfrac{
                \epsilon - t(2 + \nicefrac{\epsilon}{2})
            }{
                \nicefrac12(2 - s)^2
            }, 
            \quad
        F_3(x) - F_4(x)
            {}={}
        \tfrac{\nicefrac{\epsilon}{2} + s}{\nicefrac12(2 - s)}.
    \end{align*}
    % Plugging this into \eqref{eq:ex:Neumann:rho:1} and introducing $\bar{\beta} \coloneqq (1 - \nicefrac{s}{2})^2\beta$, it follows that
    % \begin{align*}
    %     \DRSrho
    %         {}={}& 
    %     \inf_{
    %         \substack{
    %             s,t \in [0,1],\\ 
    %             \bar{\beta} \in \R_+^4
    %         }
    %     } \;
    %     \tfrac{
    %         2(1 - \nicefrac{s}{2})^2
    %         \bigl(
    %             -st(\epsilon + \nicefrac{s}{2}) + \epsilon(s + t)
    %                 +
    %             \bar{\beta}_2 s 
    %                 +
    %             \bar{\beta}_4 t
    %         \bigr)
    %     }
    %     {
    %         \bigl(
    %             \epsilon - t(1 + \nicefrac{\epsilon}2)
    %             + 
    %             \bar{\beta}_2 - \bar{\beta}_1
    %         \bigr)^2
    %             +
    %         \bigl(
    %             (\epsilon + s)(1 - \nicefrac{s}{2})
    %             +
    %             \bar{\beta}_4 - \bar{\beta}_3
    %         \bigr)^2
    %     }
    %     \; \stt \;
    %     \inner{
    %         \bar{\beta},
    %         % x
    %         \begin{bsmallmatrix}
    %             s \\ 1-s \\ t \\ 1-t
    %         \end{bsmallmatrix}
    %         } 
    %     = 0
    % \end{align*}
    Let             
    \(
        \bar{s}
            {}\coloneqq{}
        \sqrt{\epsilon}
    \)
    and
    \(
        \bar{t}(s)
            {}\coloneqq{}
        \tfrac{\epsilon s}{s(\epsilon + s)-\epsilon}.
    \)
    Since
    $
        \inner*{ 
            F(x),
            x - x^\star
        }
            <
        0
    $
    if and only if $s \in (\bar{s}, 1]$ and $t \in (\bar{t}(s), 1]$, it suffices to take the infimum in \eqref{eq:ex:Neumann:rho:1} over this restricted domain. 
    In particular, introducing $\bar{\beta} \coloneqq \nicefrac12(2 - s)^2\beta$, it follows that
    \begin{align*}
        \DRSrho
            {}={}& 
        \inf_{
            \substack{
                s \in (\bar{s}, 1],\\
                t \in (\bar{t}(s), 1],\\ 
                \bar{\beta} \in \R_+^4
            }
        } \; 
        \tfrac{
            4(2 - s)^2
            \bigl(
                \epsilon(s + t)
                    -
                st(\epsilon + s)
                    +
                \bar{\beta}_2
                    +
                \bar{\beta}_4
            \bigr)
        }
        {
            \bigl(
                2\epsilon - t(4 + \epsilon)
                -
                2\bar{\beta}_1
                + 
                2\bar{\beta}_2
            \bigr)^2
                +
            c
            \bigl(
                (\epsilon + 2s)(2 - s)
                -
                2\bar{\beta}_3
                +
                2\bar{\beta}_4
            \bigr)^2
        }
        \; \stt \;
        \inner{
            \begin{bsmallmatrix}
                \bar{\beta}_1\\
                \bar{\beta}_2\\
                \bar{\beta}_3\\
                \bar{\beta}_4
            \end{bsmallmatrix},
            \begin{bsmallmatrix}
                s\\
                1-s\\
                t\\
                1-t
            \end{bsmallmatrix}
            } 
        = 0
    \end{align*}
    Since $s > 0$ and $t > 0$ this implies immediately that $\bar{\beta}_1 = \bar{\beta}_3 = 0$ due to the constraint.
    Furthermore, since $(\nicefrac{\epsilon}{2} + s)(2 - s) > 0$ for all $s \in (\bar{s}, 1]$, it follows immediately that $\bar{\beta}_4 = 0$ at the infimum. Furthermore, the infimum is attained, since the denominator is strictly positive.
    Finally, we claim that $\bar{\beta}_2 = 0$ at the minimum. 
    If $s \in (\bar{s}, 1)$ at the minimum, then this follows directly from the constraint.
    If $s = 1$ at the minimum, then \eqref{eq:ex:Neumann:rho:1} reduces to
    \begin{align*}
        \DRSrho
            {}={}& 
        \inf_{
            \substack{
                t \in (\epsilon, 1],\\ 
                \bar{\beta}_2 \in \R_+
            }
        } \; 
        g(t, \bar{\beta}_2)
            \coloneqq
        \tfrac{
                4(
                    \epsilon - t
                        +
                    \bar{\beta}_2
                )
        }
        {
            \bigl(
                2\epsilon - t(4 + \epsilon)
                + 
                2\bar{\beta}_2
            \bigr)^2
                +
            c
            (2 + \epsilon)^2
        },
    \end{align*}
    and the claim holds since for any $t \in (\epsilon, 1]$ the function
    $
        \R_+ \ni \bar{\beta}_2
            \mapsto                 
        g(t, \bar{\beta}_2)
    $ 
    attains its minimum at $\bar{\beta}_2 = 0$.
    % Having shown that $\bar{\beta} = 0$ at the minimum, the proof is completed by observing that the sublevel sets
    % \begin{align*}
    %     S_\alpha 
    %         {}\coloneqq{}
    %     \set{s \in (\bar{s}, 1],t \in (\bar{t}(s), 1]}[        
    %         \tfrac{
    %             4(2 - s)^2
    %             (
    %                 \epsilon(s + t) - st(\epsilon + s)
    %             )
    %         }
    %         {
    %             (
    %                 2\epsilon - t(4 + \epsilon)
    %             )^2
    %                 +
    %             (\epsilon + 2s)^2(2 - s)^2
    %         }
    %         \leq \alpha
    %     ]
    % \end{align*}
    % are convex for all $\alpha \in \R$.
\end{appendixproof}

==> TeX/Text/Proofs/SemiMonInverse.tex <==
%!TEX root = ../../../DRS-Minty.tex

% \begin{appendixproof}{prop:calculus:inverse}
%     On the one hand, if $A$ is $(\mon,\com)$\hyp{}semimonotone at $(\other{x}, \other{y})$, then \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (x, y) \in \graph A$. Hence, we equivalently have that \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (y, x) \in \graph A^{-1}$, and thus $A^{-1}$ is $(\com, \mon)$\hyp{}semimonotone at $(\other{y}, \other{x})$.
%     On the other hand, if $A^{-1}$ is $(\com, \mon)$\hyp{}semimonotone at $(\other{y}, \other{x})$, then \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (x, y) \in \graph A^{-1}$. Hence, we equivalently have that \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (y, x) \in \graph A$, and thus $A$ is $(\mon, \com)$\hyp{}semimonotone at $(\other{x},\other{y})$. The argument for (maximally) semimonotone operators is analogous. 
% \end{appendixproof}

==> TeX/Text/Proofs/gen.tex <==
%!TEX root = ../../../DRS-Minty.tex

\begin{appendixproof}{cor:sem2mon}
    % The proof is an extension of \cite[Thm. 2]{otero2011regularity} and is included for completeness.  
        Let \(H\) denote the linear mapping given by \(H(x,y)=\big(y + \xi x, \nu y + (1+ \xi\nu) x\big)\). 
        Then, it is immediate that
        \begin{align*}
            (x,y) 
                {}\in{}
            \graph A 
                {}\iff{}&
            y 
                {}\in{}
            (T - \nu \id)^{-1}x - \xi x\\
            % \dueto{(let \(\bar x = u + \xi x\))}
                {}\iff{}&
            x 
                {}\in{}
            (T- \nu \id)(y + \xi x)\\
                {}\iff{}&
            \nu y + (1+ \xi\nu) x 
                {}\in{}
            T(y + \xi x)
                {}\iff{}
            H(x,y) \in \graph T,
        \end{align*}
        % Hence, we have shown that $(x,y) \in \graph T$ if and only if $H(x,y) \in \graph A$. 
        % Note that the mapping \(H\) is invertible, such that \((x,y) = H^{-1}(r,p) = \big(p - \nu r, (1+\xi\nu)r - \xi p \big)\) where \((r,p) = H(x,y)\). 
        Note that the mapping \(H\) is invertible, with inverse \(H^{-1}(r,p) = \big(p - \nu r, (1+\xi\nu)r - \xi p \big)\). 

        Using this property, we now proceed to proof the main claim of the theorem.
        Consider pairs $(x,y), (\other{x},\other{y}) \in \graph A$ and let $(r,p) = H(x,y)$ and $(\other{r},\other{p}) = H(\other{x},\other{y})$, ensuring that \((r,p),(\other{r},\other{p})\in \graph T\).
        Operator $A$ is monotone if and only if for any $(x,y), (\other{x},\other{y}) \in \graph A$, it holds that
        \begin{align*}
            0
                {}\leq{}
            \inner{x-\other{x},y-\other{y}}
                {}={}&
            \inner{p-\nu r - \other{p} + \nu \other{r},(1+\xi\nu)r - \xi p -(1+\xi\nu)\other{r} + \xi \other{p} }\\
                {}={}&
            (1+2\xi\nu)\inner{r - \other{r},p-\other{p}} - \nu(1+\xi\nu)\nrm{r-\other{r}}^2 - \xi\nrm{p-\other{p}}^2,
            \numberthis
            \label{eq:semimon:innprod:1}
        \end{align*}
        where we used that $(x,y) = H^{-1}(r,p)$ and $(\other{x},\other{y}) = H^{-1}(\other{r},\other{p})$. Dividing both sides by $1 + 2\xi\nu$, which is positive in this case, \eqref{eq:semimon:innprod:1} may be equivalently expressed as 
        \begin{align}\label{eq:lem:calculus:inverse-sum-inverse:inequality}
            \inner{r - \other{r},p-\other{p}} 
                {}\geq{}
            % \tfrac{\monA \nu^2 + \comA (1+\xi\nu)^2 + (1+\xi\nu)\nu}{1+2\xi\nu + 2\monA \nu + 2\comA \xi (1+\xi\nu))}\nrm{r - \other{r}}^2 + \tfrac{\monA + \comA \xi^2 + \xi}{1+2\xi\nu + 2\monA \nu + 2\comA \xi (1+\xi\nu))}\nrm{p - \other{p}}^2\\
            \tfrac{\nu(1 + \xi\nu)}{1 + 2\xi\nu}\nrm{r - \other{r}}^2 + \tfrac{\xi}{1 + 2\xi\nu}\nrm{p - \other{p}}^2
        \end{align}
        Hence, the claimed equivalence between $\Bigl(\tfrac{\nu(1 + \xi\nu)}{1 + 2\xi\nu}, \tfrac{\xi}{1 + 2\xi\nu}\Bigr)$\hyp{}semimonotonicity of $T$ and monotonicity of $A$ is established. 

        % Analogous to the argument provided in the proof of \cite[Thm. 2(ii)]{otero2011regularity},
        The assertion for maximality holds since \(\graph A\) can be enlarged with a point \((\hat x,\hat y)\) without destroying monotonicity if and only if \(\graph T\) can be enlarged with \(H(\hat x,\hat y)\) without destroying \((\mon,\com)\)\hyp{}semimonotonicity (see \eqref{eq:semimon:innprod:1}).
    \end{appendixproof}

==> TeX/Text/Proofs/klee.tex <==
%!TEX root = ../../../DRS-Minty.tex

\begin{appendixproof}{lem:klee}
    \begin{proofitemize}
        \item \ref{lem:klee:LL}: Follows immediately from \cite[Prop. 4.3(ii)]{wang2010chebyshev}. 
        \item \ref{lem:klee:semi}: Let \(\varphi(s) \coloneqq -\klee_f^\alpha(s) = \inf_w h(w,s,\alpha)\) where 
        \(
            h(w,s,\alpha) \coloneqq f(w) - \tfrac{1}{2\alpha}\|w-s\|^2 + \delta_{\geq 0}(\alpha).
        \)
        As in the proof of \cite[Prop. 4.3(iii)]{wang2010chebyshev}, \(h\) is level-bounded in \(w\) locally uniformly in \((s,\alpha)\). 
        Invoke \cite[Thm. 10.13]{rockafellar2009Variational}
        to obtain that 
        \begin{align*}
            \partial(f \square \tfrac{1}{-2\alpha}\|\cdot\|^2)(s)
                {}={}
            \partial \varphi(s) 
                {}\subseteq{}  
            \bigcup_{(x_1,x_2) \in K_{f}^{\alpha}(s) } \{\tfrac{1}{-\alpha}x_1\} \cap \partial f(x_2),
                % {}={}
            % \bigcup_{x_1,x_2\in M(s)} \{\tfrac1{\rho}x_1\},
            \numberthis\label{eq:subdif:klee}
        \end{align*}
        This implies through \cite[Prop. 25.30]{bauschke2017Convex} that 
        \[
            \partial\Bigl(f \square \tfrac{1}{-2\alpha}\|\cdot\|^2\Bigr)(s) 
                {}\subseteq{}
            \partial f \Box \tfrac1{-\alpha}\id
                {}={}
            (\partial f^* - \alpha \id)^{-1}
        \]
        It then follows from \cref{cor:generation semimonotone operator} 
        % (with \(\nu=0\), \(\xi=\rho\))
        that \( \partial\Bigl(f \square \tfrac{1}{-2\alpha}\|\cdot\|^2\Bigr)\) is \((0, -\alpha)\)-semimonotone. 
        \qedhere
    \end{proofitemize}
\end{appendixproof}

==> TeX/Text/Semimonotone/Functions/Klee.tex <==
%!TEX root = ../../../../DRS-Minty.tex

\begin{definition}
    The Klee envelope of a lsc function \(f: \R^n \rightarrow \Rinf\) for $\kappa > 0$ is defined as
    \begin{equation}\label{eq:Klee}
            f^\kappa(s) 
            {}\coloneqq{}
        \sup_{w\in\R^n}\{\tfrac{1}{2\kappa}\|w-s\|^2-f(w)\}
            {}={}
        -\big(f \square \tfrac{1}{-2\kappa}\|\cdot\|^2\big)(s).
    \end{equation}
    and the associated attainment mapping is given by
    \[
        K^{\kappa}_f(s) \coloneqq \argmin_{w\in\R^n} \{f(w) - \tfrac{1}{2\kappa}\|w-s\|^2\}.
    \]
\end{definition}

We recall the following counter part of prox-boundedness \cite[Def. 4.1]{wang2010chebyshev}, which we will refer to as Klee-boundedness.
\begin{definition}
   We say that \(f:\R^n \to \Rinf\) is Klee-bounded if \(f - \tfrac{1}{2\kappa}\|\cdot\|^2\) is bounded below for some \(\kappa>0\). The infimum of all such \(\kappa\) is denoted by \(\kappa_f\) and refered to as the threshold of Klee-boundedness.  
\end{definition}

% In the next lemma we provide a semimonotonicity result for the negative of the Klee envelope, under an assumption which can be interpreted as the counter part of prox-boundedness \cite[Def. 4.1]{wang2010chebyshev}. 
\begin{lemma}[Klee envelope]\label{lem:klee}
    Let \(f:\R^n \to \Rinf\) be proper lsc convex and Klee-bounded. Let \(\kappa \in (\kappa_f, +\infty)\).
    Then, it holds that
    \begin{enumerate}
        \item \label{lem:klee:LL} \(f^\kappa\) is convex and locally Lipschitz. The mapping \(K^{\kappa}_f\) is nonempty and compact-valued.
        % \item \label{lem:klee:compact} 
        \item \label{lem:klee:semi} the subdifferential of \(-f^\kappa\) is \((0,-{\kappa})\)\hyp{}semimonotone. %(or \(\alpha\)-cohypomonotone). 
    \end{enumerate}
    \begin{proof}
        See \Cref{proof:lem:klee}
    \end{proof} 
\end{lemma}

% \begin{example}[concave function]\label{cor:strcvx}
%     Let \(f:\R^n\to \R\) be a continuous and \(\nicefrac1{\alpha}\)-strongly concave function, where $\alpha > 0$.
%     Then, \(\partial f\) is \((0,-\alpha)\)-semimonotone.
%     \begin{proof}
%         By \cite[Prop. 12.60]{rockafellar2009Variational} and strong convexity of $-f$, the conjugate $(-f)^*$ is $\alpha$\hyp{}smooth, i.e.
%         \begin{align*}
%             \inner{\nabla (-f)^*(x) - \nabla (-f)^*(\other{x}), x - \other{x}} \leq \alpha \nrm{x - \other{x}}^2, \quad \forall x, \other{x} \in \R^n.\numberthis\label{eq:cor:strcvx:1}
%         \end{align*}
%         Moreover, since $-f$ is continuous and convex, we have by 
%         \cite[Prop. 11.3]{rockafellar2009Variational} that 
%         \(
%             \nabla (-f)^* = (\partial (-f))^{-1}
%         \),
%         so that \eqref{eq:cor:strcvx:1} is equivalent to
%         \begin{align*}
%             \inner{y - \other{y}, x - \other{x}} \leq \alpha \nrm{y - \other{y}}^2, \quad \forall (x, y), (\other{x}, \other{y}) \in \graph \partial (-f).\numberthis\label{eq:cor:strcvx:2}
%         \end{align*}
%         Finally, since $-f$ is finite and convex, it follows from \cite[Cor. 9.21]{rockafellar2009Variational} that \(\partial f(\bar{x}) \subseteq - \partial (-f)(\bar{x})\), \(\forall \bar{x} \in \R^n\). Consequently, 
%         \begin{align*}
%             \inner{y - \other{y}, x - \other{x}} \geq -\alpha \nrm{y - \other{y}}^2, \quad \forall (x, y), (\other{x}, \other{y}) \in \graph \partial f \subseteq - \graph \partial (-f),
%         \end{align*}
%         which completes the proof.
%     \end{proof}
% \end{example}

% \begin{lemma}
%     Let \(h\) denote a proper lsc convex function, and let 
%     \(
%         g_\gamma \coloneqq h \circ (-\id) - \gamma^{-1}\|\cdot\|^2
%     \). Then, the Moreau envelope of \(g\) is given by
%     \(
%         g^\gamma
%             {}={}
%         \tfrac{1}{\gamma}\|\cdot\|^{2}
%             {}-{}
%         \klee_{h}^{\gamma}
%     \).
%     In particular \(g^{-\rho}\) is \((\sigma,\rho)\)-semimonotone. (? add the summation with quadratic lemma) 
% \begin{proof}
    
% Using \cite[Lemma 3.3(i),(iv)]{laude2021conjugate} it holds that for any convex function \(h\)
% \begin{align*}
%      -\klee_{h}^{\gamma}
%         {}={}
%     -\tfrac{1}{2\gamma}\|\cdot\|^{2}-\left(h\circ (\gamma \id)-\tfrac{\gamma}{2}\|\cdot\|^{2}\right)_{-}^{*}
%         {}={}
%     -\tfrac{1}{2\gamma}\|\cdot\|^{2}-\left(h\circ (-\gamma \id)-\tfrac{\gamma}{2}\|\cdot\|^{2}\right)^{*}
%  \end{align*} 
%  and for the Moreau envelope of a function \(\varphi\) it holds that 
%  \[
% \varphi^{\gamma}(x)=\tfrac{1}{2\gamma}\|\cdot\|^{2}-(\varphi\circ(\gamma\id)+\tfrac{\gamma}{2}\|\cdot\|^{2})^{*}.
%  \]
%  Setting \(\varphi =g\) it follows that 
%  \begin{align*}
%      g^\gamma 
%         {}={}
%     \tfrac{1}{2\gamma}\|\cdot\|^{2}-\left(h\circ (-\gamma \id)-\tfrac{\gamma}{2}\|\cdot\|^{2}\right)^{*}
%         {}={}
%     \tfrac{1}{\gamma}\|\cdot\|^{2}
%         {}-{}
%     \klee_{h}^{\gamma}.  
%  \end{align*}
% \end{proof}


% \end{lemma}




==> TeX/Text/Semimonotone/Functions/pseudo.tex <==
We begin by presenting a classical example of a function class which is nonconvex but satisfies the Minty assumption (corresponding to $V = 0$ in \Cref{def:SWMVI}). For additional examples, please refer to \cite{zhou2017stochastic}.
\begin{proposition}[pseudoconvex functions]\label{lem:quasiconvex}
    Let $f : \R^n \to \Rinf$ be a lsc pseudoconvex function, i.e., for all $x, \other{x} \in \R^n$ if there exists a $y \in \partial f(x)$ such that $\inner{y, \other{x}-x} \geq 0$ then $f(x) \leq f(\other{x})$.
    % \[
    %     \exists y \in \partial f(x) : \inner{y, \other{x}-x} \geq 0 \implies f(x) \leq f(\other{x}), \quad \forall x, \other{x} \in \R^n.
    % \]
    % or a continuously differentiable star-convex function, i.e.
    % \[
    %     \inner{\nabla f(x) }
    % \]
    Then, it holds that \(\partial f\) is $(0,0)$\hyp{}semimonotone at \(\set{(x^\star, 0)}[x^\star \in \zer \partial f]\), which are the global minimizers of $f$.
    \begin{proof}
        Follows by definition using \cite[Thm. 2.2(ii), Prop. 2.3(i)]{daniilidis1999subdifferentials}.
    \end{proof}
\end{proposition}

==> TeX/Text/Semimonotone/gen.tex <==
%!TEX root = ../../../DRS-Minty.tex

\begin{lemma}\label{lem:calculus:inverse-sum-inverse}
    A set-valued operator $A : \R^n \rightrightarrows \R^n$ is (maximally) $(\monA,\comA)$\hyp{}semimonotone 
    if and only if 
    for all $\xi, \nu \in \R$
    such that $\beta + 2\alpha\nu > 0$
    where
    \begin{align}\label{lem:calculus:inverse-sum-inverse:alphabeta}
        \alpha \coloneqq \xi + \monA + \comA \xi^2
        \quad \text{and} \quad
        \beta \coloneqq 1 + 2\comA\xi
    \end{align}
    it holds that
    $T = (A + \xi \id)^{-1} + \nu \id$ is (maximally) $(\mon_T,\com_T) = \bigl(\tfrac{\comA + \nu(\beta + \alpha\nu)}{\beta + 2\alpha\nu}, \tfrac{\alpha}{\beta + 2\alpha\nu}\bigr)$\hyp{}semimonotone. 
\end{lemma}



\begin{lemma}
    Let \(f : \R^n \to \Rinf\) denote a pointwise minimum of \(L_i\)-smooth functions \(f_i\), \ie, \(f(x) = \min\{f_1(x),\ldots, f_N(x)\}\). Let \(L_{\rm max} = \max_i{L_i}\), and \(\alpha> \max\{L_1,\ldots, L_N\}\), and \(c < -\tfrac{L_{\rm max}}{\alpha - L_{\rm max}}\). Then, \(\partial f\) is \((\mu_A, \rho_A)\)-semimonotone where 
    \[
        \mu_A 
        {}={}
        c \alpha,
        \quad 
        \rho_A
        {}={}
        (-\tfrac{1}{\alpha - L_{\rm max}})  \Box (\tfrac{1-c}{\alpha}).
    \]
    \begin{proof}
        Let \(\alpha > \max\{L_1,\ldots, L_N\}\). Then, by smoothness assumption \(\tfrac{\alpha}2\|\cdot\|^2 - f_i\) is \(m_i\)-convex where \(m_i \coloneqq \alpha-L_i\). Consider the decomposition of \(f\) as follows
        \[
            f(x)
            {}={}
            \varphi(x) 
            {}+{}
            \tfrac{\alpha}2\|\cdot\|^2,
            \quad 
            \varphi(x)
            {}\coloneqq{}
            \min\left\{f_1(x) - \tfrac{\alpha}2\|x\|^2,\ldots, f_N(x)-\tfrac{\alpha}2\|x\|^2\right\}.
        \]
        Being the pointwise minimum of \(m_i\)-concave functions, \(\varphi\) is itself \(\min_{i}{m_i}\) concave. By (Klee lemma) \(\varphi\) is \((0,-\tfrac1{\min_{i}{m_i}})\) semimonotone. Since \(\partial f= \partial \varphi + \alpha \id\) \cite[Ex. 8.8(c)]{Rockafellar1970Convex} it follows from \Cref{lem:sum:1} that for some \(c\in\R\) satisfying \(\tfrac{1-c}{\alpha}-\tfrac1{\min_{i}{m_i}}>0\). The latter holds for 
        \(
            c 
            {}<{}
            -\tfrac{\max_i{L_i}}{\alpha - \max_i{L_i}}
        \)

     \end{proof} 
\end{lemma}
